Understanding the role of importance weighting for deep learning

The recent paper by Byrd & Lipton (2019), based on empirical observations, raises a major concern on the impact of importance weighting for the over-parameterized deep learning models. They observe that as long as the model can separate the training data, the impact of importance weighting diminishes as the training proceeds. Nevertheless, there lacks a rigorous characterization of this phenomenon. In this paper, we provide formal characterizations and theoretical justifications on the role of importance weighting with respect to the implicit bias of gradient descent and margin-based learning theory. We reveal both the optimization dynamics and generalization performance under deep learning models. Our work not only explains the various novel phenomenons observed for importance weighting in deep learning, but also extends to the studies where the weights are being optimized as part of the model, which applies to a number of topics under active research.

==> related-work.tex <==
Importance weighting has been widely employed by deep learning studies. Causal inference for deep learning investigates heavily on the propensity score weighting method that applies the off-policy optimization with counterfactual estimator \citep{gilotte2018offline,jiang2016doubly}, modelling with observational feedback \citep{schnabel2016recommendations} and learning from controlled intervention \citep{swaminathan2015counterfactual}. The importance weights are also applied to characterize distribution shifts in such as domain adaptation \citep{azizzadenesheli2019regularized,lipton2018detecting} and learning from noisy labels \citep{song2020learning}. Other usages include curriculum learning \cite{bengio2009curriculum} and knowledge distillation \cite{hinton2015distilling} where the weights characterize the model confidence on each sample. 
\cite{byrd2019effect} first connects the observed phenomenon of importance weighting on deep learning models to the implicit bias of gradient descent \cite{soudry2018implicit}, however, they do not provide any precise characterization. 
Implicit bias of gradient descent has been observed and studied for linear model \citep{soudry2018implicit,ji2018risk}, linear neural network \citep{ji2018gradient,gunasekar2018implicit}, two-layer neural network with homogeneous activation \citep{chizat2020implicit} and smooth neural networks \citep{nacson2019lexicographic,lyu2019gradient}. The above work do not consider regularization. \cite{rosset2004margin} and \citep{wei2019regularization} studies the solution path under weak regularization, and the role of margin for the generalization of neural networks have been studied by \cite{bartlett2017spectrally,golowich2018size,neyshabur2018towards} 




